Teaching Unknown Objects by Leveraging Human Gaze and Augmented Reality in Human-Robot Interaction

Robots are becoming increasingly popular in a wide range of environments due to their exceptional work capacity, precision, efficiency, and scalability. This development has been further encouraged by advances in Artificial Intelligence, particularly Machine Learning. By employing sophisticated neural networks, robots are given the ability to detect and interact with objects in their vicinity. However, a significant drawback arises from the underlying dependency on extensive datasets and the availability of substantial amounts of training data for these object detection models. This issue becomes particularly problematic when the specific deployment location of the robot and the surroundings, are not known in advance. The vast and ever-expanding array of objects makes it virtually impossible to comprehensively cover the entire spectrum of existing objects using preexisting datasets alone. The goal of this dissertation was to teach a robot unknown objects in the context of Human-Robot Interaction (HRI) in order to liberate it from its data dependency, unleashing it from predefined scenarios. In this context, the combination of eye tracking and Augmented Reality created a powerful synergy that empowered the human teacher to communicate with the robot and effortlessly point out objects by means of human gaze. This holistic approach led to the development of a multimodal HRI system that enabled the robot to identify and visually segment the Objects of Interest in 3D space. Through the class information provided by the human, the robot was able to learn the objects and redetect them at a later stage. Due to the knowledge gained from this HRI based teaching, the robot's object detection capabilities exhibited comparable performance to state-of-the-art object detectors trained on extensive datasets, without being restricted to predefined classes, showcasing its versatility and adaptability.

==> src/head/titlepage.tex <==
\begin{titlepage}
\begin{center}


\null\vspace{0.5cm}
\makeatletter
{\huge\bfseries \@title \par}
\makeatother

\vfill
{\large \textbf{Dissertation}} \\[0.3cm]
{\large der Mathematisch-Naturwissenschaftlichen Fakult{\"a}t}\\[0.3cm]
{\large der Eberhard Karls Universit{\"a}t T{\"u}bingen}\\[0.3cm]
{\large zur Erlangung des Grades eines}\\[0.3cm]
{\large Doktors der Naturwissenschaften}\\[0.3cm]
{\large (Dr. rer. nat.)}

\vfill
vorgelegt von\\[0.3cm]
\makeatletter
{\large \@author}\\[0.3cm]
\makeatother
{\large aus T{\"u}bingen}

\vfill
{\large T{\"u}bingen}\\[0.3cm]
{\large 2023}\\[0.3cm]


\end{center}
\end{titlepage}

\thispagestyle{empty}

\mbox{}

\vfill
\noindent
\begin{flushleft}
	Gedruckt mit Genehmigung der Mathematisch-Naturwissenschaftlichen Fakult{\"a}t der Eberhard Karls Universit{\"a}t T{\"u}bingen.
\end{flushleft}
\vspace{0.5cm}

\begingroup
\renewcommand{\arraystretch}{1.3}
\setlength{\tabcolsep}{24pt} % Default value: 6pt
\noindent \begin{tabular}{@{}ll}
Tag der m\"undlichen Qualifikation:	& 02.11.2023 \\
Dekan:								& Prof.~Dr.~Thilo~Stehle \\
1.~Berichterstatterin:				& Prof.~Dr.~Enkelejda Kasneci \\
2.~Berichterstatter:				& Jun.-Prof.~Dr.~Michael Krone\\
\end{tabular}
\endgroup




==> src/tail/paper03/limitations.tex <==
\section{Limitations}
We have shown that the gaze data can be used to detect objects and their bounding boxes. What is still missing for an actual application is the combinatorial use with, e.g., a robot, which learns to detect these objects. This application, of course, still brings some challenges like inaccurate bounding boxes or wrongly detected objects. However, with a robot or a machine learning the objects, there are more possibilities like depth data and the image information from different perspectives. Thus, there are also more possibilities for optimization in this application. Another limitation of our work is that we did not perform a parameter search for the machine learning methods. This means that our results are certainly far below the possible detection rates that can be achieved. However, our results are easy to reproduce and might be considered rather as a proof-of-concept, yet conveying the potential of gaze in such tasks.
